How Good is Zero-Shot MT Evaluation for Low Resource Indian Languages?

While machine translation evaluation has been studied primarily for high-resource languages, there has been a recent interest in evaluation for low-resource languages due to the increasing availability of data and models. In this paper, we focus on a zero-shot evaluation setting focusing on low-resource Indian languages, namely Assamese, Kannada, Maithili, and Punjabi. We collect sufficient Multi-Dimensional Quality Metrics (MQM) and Direct Assessment (DA) annotations to create test sets and meta-evaluate a plethora of automatic evaluation metrics. We observe that even for learned metrics, which are known to exhibit zero-shot performance, the Kendall Tau and Pearson correlations with human annotations are only as high as 0.32 and 0.45. Synthetic data approaches show mixed results and overall do not help close the gap by much for these languages. This indicates that there is still a long way to go for low-resource evaluation.

==> discarded.tex <==
% To assess the influence of the backbone model on zero-shot performance for Indian languages, we conducted an experiment involving the COMET model. We replaced the original XLM-Roberta backbone (24 layers) with Indic-BERT v2 (12 layers), a multilingual model having 278 million parameters and trained on 23 Indian languages, including the languages in our zero-shot evaluation set.\\
% We fine-tuned COMET-model with IndicBert as backbone in two ways: 1) which regress on DA scores and then will evaluate w.r.t DA scores 2) which the model will see the MQM score, will regress on it to minimize the MSE loss and then we will evaluate it w.r.t MQM scores.
% To assess the influence of the backbone model on zero-shot performance for Indian languages, we conducted an experiment involving the COMET model. We replaced the original XLM-Roberta backbone (24 layers) with Indic-BERT v2 (12 layers), a multilingual model having 278 million parameters and trained on 23 Indian languages, including the languages in our zero-shot evaluation set.\\

% Following fine-tuning on our dedicated Indian language (IL) dataset with slightly higher learning rate of 1.0e-04, we evaluated the model's zero-shot performance. This experiment yielded positive results(shown in row "indicBert-DA and "IndicBert-MQM" in Table \autoref{tab:corr_formula_metrics}), demonstrating that fine-tuning with an Indian-specific model like Indic-BERT v2, which had prior exposure to these languages, led to an improvement in zero-shot performance.

% We use COMET-DA for our experiments with synthetic dataset, as it is the best performing model for IL languages and also it has not seen low-resource languages.\\
% We have created synthetic data for all four zero shot language(assamese, maithili, Kannada, Punjabi), and in every experiment we fine-tuned COMET-DA by taking synthetic data of one particular language and later evaluate that model for that one language only. The details of hyperparameters used is shared in \autoref{sec:appendix_synthetic} 
% To assess the efficacy of synthetic data, we categorized our experiments into three groups: \\
% 1) Single stage: In this approach, we integrated our synthetic data with the IL dataset in different proportions starting from 5K examples( equal proportions) and subsequently fine-tuned the model.\\
% 2) Two-stage (synthetic preceding real): Here, we initially fine-tuned the model on the synthetic dataset of a particular language that we want to evaluate, followed by a second stage where we utilized the checkpoints from the initial fine-tuning and conducted further fine-tuning on IL dataset with a slightly reduced learning rate.\\
% 3) Two-stage (real preceding synthetic): Opposite to the above specified setup, in this fine-tuned the model on the IL dataset first, followed by further fine-tuning on synthetic dataset of particular language with a slightly reduced learning rate.\\

In this work, we investigated the potential of synthetic data for improving COMET-DA's performance on unseen low-resource languages. This choice was based on COMET-DA's superior performance on Indian languages and its lack of exposure to the target low-resource languages.
We constructed synthetic datasets for four target languages (Assamese, Maithili, Kannada, and Punjabi). In each experiment, we fine-tuned COMET-DA using the synthetic data of a specific language and evaluated its performance on that same language only. Details regarding hyperparameter settings are provided in  \ref{sec:appendix_synthetic}.
We categorized our experiments into three groups: \\
1) Single stage: In this approach, we integrated our synthetic data with the IL dataset in different proportions starting from 5K examples and subsequently fine-tuned the model.\\
2) Two-stage (synthetic preceding real): Here, we initially fine-tuned the model on the synthetic dataset of a particular language that we want to evaluate, followed by a second stage where we utilized the checkpoints from the initial fine-tuning and conducted further fine-tuning on IL dataset with a slightly reduced learning rate.\\
3) Two-stage (real preceding synthetic): Conversely, in this fine-tuned the model on the IL dataset first, followed by further fine-tuning on synthetic dataset of particular language with a slightly reduced learning rate.\\

While all three approaches incorporated synthetic data, none conclusively outperformed the baseline models (COMET-DA and Indic-COMET-DA). The Single-Stage approach showed modest improvement with equal proportions of real and synthetic data, but performance declined with more synthetic data. Overall, these experiments yielded mixed results, raising questions about the effectiveness of using increasing amounts of synthetic data for low-resource language translation tasks.

==> instructions.tex <==
\section{Engines}

To produce a PDF file, pdf\LaTeX{} is strongly recommended (over original \LaTeX{} plus dvips+ps2pdf or dvipdf). Xe\LaTeX{} also produces PDF files, and is especially suitable for text in non-Latin scripts.
\begin{table}
\centering
\begin{tabular}{lc}
\hline
\textbf{Command} & \textbf{Output}\\
\hline
\verb|{\"a}| & {\"a} \\
\verb|{\^e}| & {\^e} \\
\verb|{\`i}| & {\`i} \\ 
\verb|{\.I}| & {\.I} \\ 
\verb|{\o}| & {\o} \\
\verb|{\'u}| & {\'u}  \\ 
\verb|{\aa}| & {\aa}  \\\hline
\end{tabular}
\begin{tabular}{lc}
\hline
\textbf{Command} & \textbf{Output}\\
\hline
\verb|{\c c}| & {\c c} \\ 
\verb|{\u g}| & {\u g} \\ 
\verb|{\l}| & {\l} \\ 
\verb|{\~n}| & {\~n} \\ 
\verb|{\H o}| & {\H o} \\ 
\verb|{\v r}| & {\v r} \\ 
\verb|{\ss}| & {\ss} \\
\hline
\end{tabular}
\caption{Example commands for accented characters, to be used in, \emph{e.g.}, Bib\TeX{} entries.}
\label{tab:accents}
\end{table}
\section{Preamble}
\begin{table*}
\centering
\begin{tabular}{lll}
\hline
\textbf{Output} & \textbf{natbib command} & \textbf{Old ACL-style command}\\
\hline
\citep{ct1965} & \verb|\citep| & \verb|\cite| \\
\citealp{ct1965} & \verb|\citealp| & no equivalent \\
\citet{ct1965} & \verb|\citet| & \verb|\newcite| \\
\citeyearpar{ct1965} & \verb|\citeyearpar| & \verb|\shortcite| \\
\citeposs{ct1965} & \verb|\citeposs| & no equivalent \\
\citep[FFT;][]{ct1965} &  \verb|\citep[FFT;][]| & no equivalent\\
\hline
\end{tabular}
\caption{\label{citation-guide}
Citation commands supported by the style file.
The style is based on the natbib package and supports all natbib citation commands.
It also supports commands defined in previous ACL style files for compatibility.
}
\end{table*}
The first line of the file must be
\begin{quote}
\begin{verbatim}
\documentclass[11pt]{article}
\end{verbatim}
\end{quote}
To load the style file in the review version:
\begin{quote}
\begin{verbatim}
\usepackage[review]{ACL2023}
\end{verbatim}
\end{quote}
For the final version, omit the \verb|review| option:
\begin{quote}
\begin{verbatim}
\usepackage{ACL2023}
\end{verbatim}
\end{quote}
To use Times Roman, put the following in the preamble:
\begin{quote}
\begin{verbatim}
\usepackage{times}
\end{verbatim}
\end{quote}
(Alternatives like txfonts or newtx are also acceptable.)
Please see the \LaTeX{} source of this document for comments on other packages that may be useful.
Set the title and author using \verb|\title| and \verb|\author|. Within the author list, format multiple authors using \verb|\and| and \verb|\And| and \verb|\AND|; please see the \LaTeX{} source for examples.
By default, the box containing the title and author names is set to the minimum of 5 cm. If you need more space, include the following in the preamble:
\begin{quote}
\begin{verbatim}
\setlength\titlebox{<dim>}
\end{verbatim}
\end{quote}
where \verb|<dim>| is replaced with a length. Do not set this length smaller than 5 cm.

\section{Document Body}

\subsection{Footnotes}

Footnotes are inserted with the \verb|\footnote| command.\footnote{This is a footnote.}

\subsection{Tables and figures}

See Table~\ref{tab:accents} for an example of a table and its caption.
\textbf{Do not override the default caption sizes.}

\subsection{Hyperlinks}

Users of older versions of \LaTeX{} may encounter the following error during compilation: 
\begin{quote}
\tt\verb|\pdfendlink| ended up in different nesting level than \verb|\pdfstartlink|.
\end{quote}
This happens when pdf\LaTeX{} is used and a citation splits across a page boundary. The best way to fix this is to upgrade \LaTeX{} to 2018-12-01 or later.

\subsection{Citations}



Table~\ref{citation-guide} shows the syntax supported by the style files.
We encourage you to use the natbib styles.
You can use the command \verb|\citet| (cite in text) to get ``author (year)'' citations, like this citation to a paper by \citet{Gusfield:97}.
You can use the command \verb|\citep| (cite in parentheses) to get ``(author, year)'' citations \citep{Gusfield:97}.
You can use the command \verb|\citealp| (alternative cite without parentheses) to get ``author, year'' citations, which is useful for using citations within parentheses (e.g. \citealp{Gusfield:97}).

\subsection{References}

\nocite{Ando2005,augenstein-etal-2016-stance,andrew2007scalable,rasooli-tetrault-2015,goodman-etal-2016-noise,harper-2014-learning}

The \LaTeX{} and Bib\TeX{} style files provided roughly follow the American Psychological Association format.
If your own bib file is named \texttt{custom.bib}, then placing the following before any appendices in your \LaTeX{} file will generate the references section for you:
\begin{quote}
\begin{verbatim}
\bibliographystyle{acl_natbib}
\bibliography{custom}
\end{verbatim}
\end{quote}
You can obtain the complete ACL Anthology as a Bib\TeX{} file from \url{https://aclweb.org/anthology/anthology.bib.gz}.
To include both the Anthology and your own .bib file, use the following instead of the above.
\begin{quote}
\begin{verbatim}
\bibliographystyle{acl_natbib}
\bibliography{anthology,custom}
\end{verbatim}
\end{quote}
Please see Section~\ref{sec:bibtex} for information on preparing Bib\TeX{} files.

\subsection{Appendices}

Use \verb|\appendix| before any appendix section to switch the section numbering over to letters. See Appendix~\ref{sec:appendix} for an example.

\section{Bib\TeX{} Files}
\label{sec:bibtex}

Unicode cannot be used in Bib\TeX{} entries, and some ways of typing special characters can disrupt Bib\TeX's alphabetization. The recommended way of typing special characters is shown in Table~\ref{tab:accents}.

Please ensure that Bib\TeX{} records contain DOIs or URLs when possible, and for all the ACL materials that you reference.
Use the \verb|doi| field for DOIs and the \verb|url| field for URLs.
If a Bib\TeX{} entry has a URL or DOI field, the paper title in the references section will appear as a hyperlink to the paper, using the hyperref \LaTeX{} package.

\section*{Limitations}
ACL 2023 requires all submissions to have a section titled ``Limitations'', for discussing the limitations of the paper as a complement to the discussion of strengths in the main text. This section should occur after the conclusion, but before the references. It will not count towards the page limit.
The discussion of limitations is mandatory. Papers without a limitation section will be desk-rejected without review.

While we are open to different types of limitations, just mentioning that a set of results have been shown for English only probably does not reflect what we expect. 
Mentioning that the method works mostly for languages with limited morphology, like English, is a much better alternative.
In addition, limitations such as low scalability to long text, the requirement of large GPU resources, or other things that inspire crucial further investigation are welcome.

\section*{Ethics Statement}
Scientific work published at ACL 2023 must comply with the ACL Ethics Policy.\footnote{\url{https://www.aclweb.org/portal/content/acl-code-ethics}} We encourage all authors to include an explicit ethics statement on the broader impact of the work, or other ethical considerations after the conclusion but before the references. The ethics statement will not count toward the page limit (8 pages for long, 4 pages for short papers).

\section*{Acknowledgements}
This document has been adapted by Jordan Boyd-Graber, Naoaki Okazaki, Anna Rogers from the style files used for earlier ACL, EMNLP and NAACL proceedings, including those for
EACL 2023 by Isabelle Augenstein and Andreas Vlachos,
EMNLP 2022 by Yue Zhang, Ryan Cotterell and Lea Frermann,
ACL 2020 by Steven Bethard, Ryan Cotterell and Rui Yan,
ACL 2019 by Douwe Kiela and Ivan Vuli\'{c},
NAACL 2019 by Stephanie Lukin and Alla Roskovskaya, 
ACL 2018 by Shay Cohen, Kevin Gimpel, and Wei Lu, 
NAACL 2018 by Margaret Mitchell and Stephanie Lukin,
Bib\TeX{} suggestions for (NA)ACL 2017/2018 from Jason Eisner,
ACL 2017 by Dan Gildea and Min-Yen Kan, NAACL 2017 by Margaret Mitchell, 
ACL 2012 by Maggie Li and Michael White, 
ACL 2010 by Jing-Shin Chang and Philipp Koehn, 
ACL 2008 by Johanna D. Moore, Simone Teufel, James Allan, and Sadaoki Furui, 
ACL 2005 by Hwee Tou Ng and Kemal Oflazer, 
ACL 2002 by Eugene Charniak and Dekang Lin, 
and earlier ACL and EACL formats written by several people, including
John Chen, Henry S. Thompson and Donald Walker.
Additional elements were taken from the formatting instructions of the \emph{International Joint Conference on Artificial Intelligence} and the \emph{Conference on Computer Vision and Pattern Recognition}.

==> new_tab_res_synthetic.tex <==
\begin{table*}[t!]
\footnotesize
\small 
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{l|cc|cc|cc|cc|cc}
\toprule
             & \multicolumn{2}{c|}{\bf asm} & \multicolumn{2}{c|}{\bf mai} & \multicolumn{2}{c|}{\bf kan} & \multicolumn{2}{c|}{\bf pan} & \multicolumn{2}{c|}{\bf Average} \\
\multirow{-2}{*} {\bf Metric}      & $\tau$          & $\rho$          & $\tau$          & $\rho$           & $\tau$          & 	$\rho$           & $\tau$          & $\rho$           & $\tau$          & $\rho$        \\ 
\midrule
 COMET-DA      & 0.228      & 0.298      & 0.172      & 0.264      & 0.281      & 0. 390     & 0.300      & 0.358      & 0.245      & 0.328           \\
Indic-COMET-DA   & 0.263      & 0.348      & 0.221      & 0.3      & 0.353      & 0.511      & 0.293      & 0.361      & 0.283      & 0.38           \\

\midrule
% \multirow{3}{8em} {\raisebox{-.2in}{\rotatebox{90}{Stage-1}}}  &   &   & & & & &  & &       & \\
% \renewcommand\arraystretch{1.2}
Stage-1 x  & 0.232  & 0.348    & 0.337   & 0.473   & 0.279    & 0.437   & 0.305    & 0.378     & 0.288      & 0.409           \\
% Stage-1 2*x &  0.242 & 0.367    & 0.333   & 0.472    & 0.233    & 0.368   &   -    &  -     & -      & -           \\
% Stage-1 4*x & 0.196  & 0.293    & 0.336   & 0.425    & 0.232    & 0.358   &   -    &  -     & -      &  -          \\
\midrule

Stage-2 S/R-x &   0.234  &  0.345    & 0.264   & 0.360    & 0.325    & 0.497   & 0.297    & 0.377     & 0.280      & 0.395           \\
% Stage-2 S/R-2*x  &   0.248  &   0.355    & 0.278   & 0.384    & 0.32 &  0.504   &   -    &  -     & -      & -           \\
% Stage-2 S/R-4*x  &  0.265  & 0.381    & 0.300   & 0.429    & 0.308    & 0.485   &   -    &  -     & -      & -     \\
\midrule

Stage-2 R/S-x   & 0.194  & 0.292   & 0.211   & 0.322    & 0.325    & 0.463   & 0.279    & 0.342     & 0.252   & 0.355          \\
% Stage-2 R/S-2*x & 0.160  & 0.251    & 0.225   & 0.345   & 0.316   &  0.442   &   -    &  -     & -      & -      \\
% Stage-2 R/S-4*x & 0.167  & 0.252    & 0.206   & 0.303    & 0.335    & 0.410   &   -    &  -     & -      & -           \\
 
% \midrule
% %EA          & 0.331      & 0.181      & 0.086      & 0.066      & 0.143      & 0.054      & 0.397      & 0.301      & 0.203      & 0.149      & 0.232       & 0.150      \\
% %VE          & 0.380      & 0.265      & \bf 0.274      & \bf 0.183      & 0.234      & 0.153      & 0.412      & 0.331      & 0.337      & 0.227      & 0.327       & 0.232      \\
% %GM          & 0.394      & 0.266      & 0.234      & 0.162      & 0.241      & 0.147      & \bf 0.426      & \bf 0.338      & \bf 0.382      & 0.264      & 0.335       & 0.235      \\
% LASER embs  & 0.097      & 0.191      & 0.119      & 0.306      & 0.139      & 0.275      & 0.036      & 0.042      & 0.098      & 0.204      \\
% LabSE embs  & \bf 0.128      & \bf 0.194      & 0.125      & 0.169      & \bf 0.219      & \bf 0.366      & 0.19      & 0.303      & 0.166      & \bf 0.258         \\
% \midrule
% mBERT       & 0.131      & 0.247      & 0.212      & 0.388      & \bf 0.165      & \bf 0.248      & 0.234      & 0.281      & 0.186      & 0.291           \\
% distilmBERT & 139      & 0.267      & 0.25      & 0.416      & 0.169      & 0.263      & \bf 0.245      & \bf 0.306      & \bf 0.201      & 0.313     \\
% IndicBERT   & 0.199      & 0.29      & 0.235      & 0.389      & 0.191      & 0.276      & 0.237      & 0.311      & 0.216      & 0.317         \\
% MuRIL       & \bf 0.206      & \bf 0.324      & \bf 0.309      & \bf 0.476      & 0.162      & 0.239      & 0.204      & 0.269      & 0.220      & \bf 0.327     \\
% \midrule
% %PRISM       & 0.114      & 0.024      & 0.178      & 0.124      & 0.131      & 0.084      & 0.089      & 0.064      & -0.040     & -0.040     & 0.094       & 0.051      \\
% BLEURT-20   & 0.119      & 0.185      & 0.32      & 0.44      & 0.279      & 0.488      & 0.28      & 0.352      & 0.250      & 0.366            \\

% COMET-QE-DA 
% & 0.417 & 0.324 
% & 0.535 & \bf 0.404
% & 0.551 & 0.430
% & 0.386 & 0.341
% &0.531 & 0.391 
% & 0.414 & 0.378\\


% COMET-QE-MQM 
% & 0.387 & 0.309
% & 0.590 & 0.403
% & 0.577 & 0.392 
% & 0.438 & 0.392
% & 0.571 & 0.399
% & 0.513 & 0.379
% \\

% COMET-DA    & \bf 0.557     & \bf 0.403     & \bf 0.581     & 0.390     &  0.426    &  0.306      & \textbf{0.531}      & \textbf{0.419}      &  0.529      &  0.412      & 0.525      & 0.386      \\

% COMET-MQM   & 0.465    & 0.360      & 0.529      &   0.370    &  \bf 0.686     &  \bf 0.459   & 0.508       &   0.392    & \bf 0.597     & \bf  0.432    & \bf 0.557      & \bf 0.402     \\

% Indic-COMET-MQM        &  0.548      & \bf 0.420     & \bf 0.631      & \bf 0.426    & \bf 0.471         & \bf 0.332   &  0.502      &  0.409     & \bf 0.590      & \bf 0.447     \\
\bottomrule
\end{tabular}
}
\caption{
KendallTau ($\tau$) and Pearson($\rho$) correlation scores of experiments with synthetic data. First block consists of COMET-DA and Indic-COMET-DA models, followed by the results of different stages of synthetic data. Here, x =5000 means 5K examples of synthetic data is added in fine-tuning process. For example, Stage-2 S/R-4*x shows the stage-2 result of a particular language, in which COMET-DA is first fine-tuned on synthetic data of size 4*x i.e. 20k, followed by real data. Detailed can be found in appendix \ref{tab:synthetic_result_appendix}  }
\label{tab:res_synthetic_result}
\end{table*}

==> old_ft_related_lang.tex <==
\begin{table*}[t!]
\footnotesize
\small 
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{l|cc|cc|cc|cc|cc}
\toprule
            & \multicolumn{2}{c|}{\bf asm} & \multicolumn{2}{c|}{\bf mai} & \multicolumn{2}{c|}{\bf kan} & \multicolumn{2}{c|}{\bf pan} & \multicolumn{2}{c|}{\bf Average} \\
\multirow{-2}{*}{\bf Metric}      & $\tau$          & $\rho$          & $\tau$          & $\rho$           & $\tau$          & 	$\rho$           & $\tau$          & $\rho$           & $\tau$          & $\rho$        \\ 
% \midrule
% COMET-DA      & 0.228      & 0.298      & 0.172      & 0.264      & 0.281      & 0. 390     & 0.300      & 0.358      & 0.245      & 0.328           \\
% COMET-MQM      & 0.26      & 0.381     & 0.199      & 0.291     & 0.290      & 0.410      & 0.266      & 0.334      & 0.254      & 0.354          \\
% COMET-QE-DA      & 0.29      & 0.34      & 0.08      & 0.07      & 0.3      & 0.45      & 0.27      & 0.33      & 0.235      & 0.298          \\
% COMET-QE-MQM      & 0.23      & 0.35      & 0.13      & 0.2      & 0.3      & 0.44      & 0.22      & 0.29      & 0.22      & 0.32          \\
\midrule
 Indic-COMET-DA   & 0.263      & 0.348      & 0.221      & 0.3      & 0.353      & 0.511      & \bf0.293      & \bf0.361      & 0.283      & 0.38           \\
 Indic-COMET-MQM    & 0.201     & 0.270     & 0.201      & 0.288      & 0.251      & 0.388      & 0.282      & 0.340      & 0.234      & 0.322         \\
Base-IndicBERT(DA)      &  0.273      &  0.396      & \bf 0.380      &  \bf0.552      & \bf 0.384      & \bf 0.528      &  0.259     &  0.353      & \bf 0.324      & \bf 0.457         \\
Base-IndicBERT(MQM)         & \bf0.293      & \bf0.426      & 0.311      & 0.483      & 0.302      & 0.44      & 0.224      & 0.313      & 0.283      & 0.416        \\

%  \midrule
% Indic-COMET-QE-DA   & 0.075      & 0.104      & 0.199      & 0.265      & 0.103      & 0.155      & 0.098      & 0.154      & 0.119      & 0.170            \\
% Indic-COMET-QE-MQM    & 0.201     & 0.270     & 0.201      & 0.288      & 0.251      & 0.388      & 0.282      & 0.340      & 0.234      & 0.322         \\
% IndicBERT-QE(DA)      &  0.273      &  0.396      &  0.380      &  0.552      &  0.384      &  0.528      &  0.259     &  0.353      & \bf 0.324      & \bf 0.457         \\
% IndicBERT-QE(mqm)         & 0.293      & 0.426      & 0.311      & 0.483      & 0.302      & 0.44      & 0.224      & 0.313      & 0.283      & 0.416        \\

\bottomrule
\end{tabular}
}
\caption{Segment-level Pearson ($\rho$) and Kendall tau ($\tau$) correlations of the finetuned version of the best publicly available COMET variant with default XLM-Roberta backbone and InicBERT backbone.}
\label{tab:indic_trained_metrics_corrs}
\end{table*}

==> old_gemba_mqm.tex <==
\begin{table*}[t!]
\footnotesize
\small 
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{l|cc|cc|cc|cc|cc}
\toprule
            & \multicolumn{2}{c|}{\bf asm} & \multicolumn{2}{c|}{\bf mai} & \multicolumn{2}{c|}{\bf kan} & \multicolumn{2}{c|}{\bf pan} & \multicolumn{2}{c|}{\bf Average} \\
\multirow{-2}{*}{\bf Metric}      & $\tau$          & $\rho$          & $\tau$          & $\rho$           & $\tau$          & 	$\rho$           & $\tau$          & $\rho$           & $\tau$          & $\rho$        \\ 
\midrule
GEMBA-MQM      & 0.235      & 0.266      & 0.085      & 0.118      & 0.108      & 0.079     & 0.282      & 0.235      & -      & -           \\
GEMBA-MQM(IL lang)      & 0.228      & 0.276     & 0.081      & 0.077     & 0.05      & 0.069      & 0.171      & 0.261      & -      & -          \\
% COMET-QE-DA      & 0.29      & 0.34      & 0.08      & 0.07      & 0.3      & 0.45      & 0.27      & 0.33      & 0.235      & 0.298          \\
% COMET-QE-MQM      & 0.23      & 0.35      & 0.13      & 0.2      & 0.3      & 0.44      & 0.22      & 0.29      & 0.22      & 0.32          \\
% \midrule

% Indic-COMET-DA   & 0.263      & 0.348      & 0.221      & 0.3      & 0.353      & 0.511      & 0.293      & 0.361      & 0.283      & 0.38           \\
% Indic-COMET-MQM    & 0.201     & 0.270     & 0.201      & 0.288      & 0.251      & 0.388      & 0.282      & 0.340      & 0.234      & 0.322         \\
% IndicBERT(DA)      &  0.273      &  0.396      &  0.380      &  0.552      &  0.384      &  0.528      &  0.259     &  0.353      & \bf 0.324      & \bf 0.457         \\
% IndicBERT(mqm)         & 0.293      & 0.426      & 0.311      & 0.483      & 0.302      & 0.44      & 0.224      & 0.313      & 0.283      & 0.416        \\
%  \midrule

\bottomrule
\end{tabular}
}
\caption{Segment-level Pearson ($\rho$) and Kendall tau ($\tau$) correlations of GEMBA-MQM.}
\label{tab:indic_trained_metrics_corrs}
\end{table*}

==> old_seg_level_corrs.tex <==
\begin{table*}[t!]
\footnotesize
\small 
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{l|cc|cc|cc|cc|cc}
\toprule
            & \multicolumn{2}{c|}{\bf asm} & \multicolumn{2}{c|}{\bf mai} & \multicolumn{2}{c|}{\bf kan} & \multicolumn{2}{c|}{\bf pan} & \multicolumn{2}{c|}{\bf Average} \\
\multirow{-2}{*}{\bf Metric}      & $\tau$          & $\rho$          & $\tau$          & $\rho$           & $\tau$          & 	$\rho$           & $\tau$          & $\rho$           & $\tau$          & $\rho$        \\ 
\midrule
BLEU 1      & 0.063      & 0.072      & -0.131      & -0.047      & -0.017      & -0.046      & -0.002      & -0.162      & -0.022      & -0.046           \\
BLEU 2      & 0.058      & 0.081      & 0.078      & -0.028      & 0.016      & 0.035      & -0.016      & 0.065      & 0.034      & 0.038          \\
BLEU 3      & 0.020      & 0.036      & -0.028      & -0.072      & 0.111      & 0.061      & -0.055      & 0.023      & 0.012      & 0.012          \\
BLEU 4      & 0.001      & 0.026      & -0.032      & -0.036      & -0.088      & -0.110      & -0.023      & 0.065      & -0.036      & -0.014          \\
SacreBLEU   & 0.075      & 0.104      & 0.199      & 0.265      & 0.103      & 0.155      & 0.098      & 0.154      & 0.119      & 0.170            \\
ROUGE-L     & 0.088      & 0.128      & 0.052      & 0.055      & 0.005      & 0.003      & -0.074      & 0.065      & 0.018      & 0.063         \\
chrF++      & \bf 0.160      & \bf 0.254      & \bf 0.252      & \bf 0.366      & \bf 0.145      & \bf 0.228      & \bf 0.164     & \bf 0.255      & \bf 0.180      & \bf 0.276         \\
TER         & 0.123      & 0.158      & 0.257      & 0.403      & 0.131      & 0.199      & 0.17      & 0.24      & 0.17      & 0.25        \\
\midrule
%EA          & 0.331      & 0.181      & 0.086      & 0.066      & 0.143      & 0.054      & 0.397      & 0.301      & 0.203      & 0.149      & 0.232       & 0.150      \\
%VE          & 0.380      & 0.265      & \bf 0.274      & \bf 0.183      & 0.234      & 0.153      & 0.412      & 0.331      & 0.337      & 0.227      & 0.327       & 0.232      \\
%GM          & 0.394      & 0.266      & 0.234      & 0.162      & 0.241      & 0.147      & \bf 0.426      & \bf 0.338      & \bf 0.382      & 0.264      & 0.335       & 0.235      \\
LASER embs  & 0.097      & 0.191      & 0.119      & 0.306      & 0.139      & 0.275      & 0.036      & 0.042      & 0.098      & 0.204      \\
LabSE embs  & \bf 0.128      & \bf 0.194      & 0.125      & 0.169      & \bf 0.219      & \bf 0.366      & 0.19      & 0.303      & 0.166      & \bf 0.258         \\
\midrule
mBERT       & 0.131      & 0.247      & 0.212      & 0.388      & \bf 0.165      & \bf 0.248      & 0.234      & 0.281      & 0.186      & 0.291           \\
distilmBERT & 139      & 0.267      & 0.25      & 0.416      & 0.169      & 0.263      & \bf 0.245      & \bf 0.306      & \bf 0.201      & 0.313     \\
IndicBERT   & 0.199      & 0.29      & 0.235      & 0.389      & 0.191      & 0.276      & 0.237      & 0.311      & 0.216      & 0.317         \\
MuRIL       & \bf 0.206      & \bf 0.324      & \bf 0.309      & \bf 0.476      & 0.162      & 0.239      & 0.204      & 0.269      & 0.220      & \bf 0.327     \\
\midrule
%PRISM       & 0.114      & 0.024      & 0.178      & 0.124      & 0.131      & 0.084      & 0.089      & 0.064      & -0.040     & -0.040     & 0.094       & 0.051      \\
BLEURT-20   & 0.119      & 0.185      & 0.32      & 0.44      & 0.279      & 0.488      & 0.28      & 0.352      & 0.250      & 0.366            \\
COMET-DA      & 0.228      & 0.298      & 0.172      & 0.264      & 0.281      & 0. 390     & 0.300      & 0.358      & 0.245      & 0.328           \\
COMET-MQM      & 0.26      & 0.381     & 0.199      & 0.291     & 0.290      & 0.410      & 0.266      & 0.334      & 0.254      & 0.354          \\
COMET-QE-DA      & 0.29      & 0.34      & 0.08      & 0.07      & 0.3      & 0.45      & 0.27      & 0.33      & 0.235      & 0.298          \\
COMET-QE-MQM      & 0.23      & 0.35      & 0.13      & 0.2      & 0.3      & 0.44      & 0.22      & 0.29      & 0.22      & 0.32          \\
COMET-Kiwi      & 0.344      & 0.475      & 0.115      & 0.129      & 0.371      & 0.514      & 0.322      & 0.392      & 0.288      & 0.3775          \\
COMET-Kiwi-xl      & 0.334      & 0.48      & 0.3      & 0.338      & 0.337      & 0.486      & 0.266      & 0.352      & 0.309      & 0.414          \\



% COMET-QE-DA 
% & 0.417 & 0.324 
% & 0.535 & \bf 0.404
% & 0.551 & 0.430
% & 0.386 & 0.341
% &0.531 & 0.391 
% & 0.414 & 0.378\\


% COMET-QE-MQM 
% & 0.387 & 0.309
% & 0.590 & 0.403
% & 0.577 & 0.392 
% & 0.438 & 0.392
% & 0.571 & 0.399
% & 0.513 & 0.379
% \\

% COMET-DA    & \bf 0.557     & \bf 0.403     & \bf 0.581     & 0.390     &  0.426    &  0.306      & \textbf{0.531}      & \textbf{0.419}      &  0.529      &  0.412      & 0.525      & 0.386      \\

% COMET-MQM   & 0.465    & 0.360      & 0.529      &   0.370    &  \bf 0.686     &  \bf 0.459   & 0.508       &   0.392    & \bf 0.597     & \bf  0.432    & \bf 0.557      & \bf 0.402     \\

% Indic-COMET-MQM        &  0.548      & \bf 0.420     & \bf 0.631      & \bf 0.426    & \bf 0.471         & \bf 0.332   &  0.502      &  0.409     & \bf 0.590      & \bf 0.447     \\
\bottomrule
\end{tabular}
}
\caption{Segment-level Pearson ($\rho$) and Kendall tau ($\tau$) correlations of different metrics. The best metric correlation amongst each metric category \cite{sai2022survey} in \textbf{bold}. We observe that COMET-MQM is the best-performing metric overall for all languages in consideration. All correlations are significant ($p< 0.05$).}
\label{tab:corr_formula_metrics}
\end{table*}

==> tab_old_langs.tex <==
\begin{table*}[t!]
\footnotesize
\small 
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{l|cc|cc|cc|cc|cc|cc}
\toprule
            & \multicolumn{2}{c|}{\bf gu} & \multicolumn{2}{c|}{\bf hi} & \multicolumn{2}{c|}{\bf mr} & \multicolumn{2}{c|}{\bf ml} & \multicolumn{2}{c|}{\bf ta} & \multicolumn{2}{c}{\bf Average} \\
\multirow{-2}{*}{\bf Metric}      & $\rho$          & $\tau$           & $\rho$          & $\tau$           & $\rho$          & 	$\tau$           & $\rho$          & $\tau$           & $\rho$          & $\tau$          & $\rho$           & $\tau$           \\ 
\midrule
BLEU 1      & 0.364      & 0.255      & 0.266      & 0.187      & 0.228      & 0.148      & 0.393      & 0.331      & 0.316      & 0.213      & 0.314       & 0.227      \\
BLEU 2      & 0.329      & 0.247      & 0.280      & 0.192      & 0.190      & 0.135      & 0.331      & 0.302      & 0.291      & 0.205      & 0.284       & 0.216      \\
BLEU 3      & 0.294      & 0.234      & 0.265      & 0.186      & 0.134      & 0.119      & 0.250      & 0.271      & 0.227      & 0.182      & 0.234       & 0.198      \\
BLEU 4      & 0.235      & 0.215      & 0.245      & 0.171      & 0.091      & 0.103      & 0.180      & 0.246      & 0.171      & 0.168      & 0.184       & 0.181      \\
SacreBLEU   & 0.293      & 0.239      & 0.255      & 0.168      & 0.164      & 0.132      & 0.274      & 0.298      & 0.244      & 0.189      & 0.246       & 0.205      \\
ROUGE-L     & 0.350      & 0.251      & 0.295      & 0.204      & 0.206      & 0.132      & 0.376      & 0.322      & 0.308      & 0.206      & 0.307       & 0.223      \\
chrF++      & \bf 0.408      & \bf 0.287      & \bf 0.299      & \bf 0.205      & 0\bf .260      & \bf 0.170      & \bf 0.411      & \bf 0.338      & \bf 0.361      & \bf 0.250      & \bf 0.348       & \bf 0.250      \\
TER         & 0.304      & 0.237      & 0.263      & 0.196      & 0.203      & 0.135      & 0.343      & 0.307      & 0.272      & 0.199      & 0.277       & 0.215      \\
\midrule
EA          & 0.331      & 0.181      & 0.086      & 0.066      & 0.143      & 0.054      & 0.397      & 0.301      & 0.203      & 0.149      & 0.232       & 0.150      \\
VE          & 0.380      & 0.265      & \bf 0.274      & \bf 0.183      & 0.234      & 0.153      & 0.412      & 0.331      & 0.337      & 0.227      & 0.327       & 0.232      \\
GM          & 0.394      & 0.266      & 0.234      & 0.162      & 0.241      & 0.147      & \bf 0.426      & \bf 0.338      & \bf 0.382      & 0.264      & 0.335       & 0.235      \\
LASER embs  & 0.094      & 0.156      & 0.135      & 0.123      & 0.159      & 0.069      & 0.357      & 0.295      & 0.126      & 0.099      & 0.174       & 0.148      \\
LabSE embs  & \bf 0.504      & \bf 0.319      & 0.149      & 0.185      & \bf 0.319      & \bf 0.204      & 0.416      & 0.337      & 0.339      & \bf 0.286      & \bf 0.345       & \bf 0.266      \\
\midrule
mBERT       & 0.448      & 0.297      & 0.337      & 0.231      & \bf 0.301      & \bf 0.194      & 0.462      & 0.367      & 0.413      & 0.281      & 0.392       & 0.274      \\
distilmBERT & 0.431      & 0.289      & 0.316      & 0.220      & 0.281      & 0.181      & \bf 0.465      & \bf 0.371      & \bf 0.415      & 0.278      & 0.382       & 0.268      \\
IndicBERT   & 0.456      & 0.308      & 0.346      & 0.235      & 0.281      & 0.182      & 0.440      & 0.357      & 0.402      & 0.282      & 0.385       & 0.273      \\
MuRIL       & \bf 0.465      & \bf 0.322      & \bf 0.353      & \bf 0.243      & 0.292      & 0.184      & 0.449      & 0.369      & 0.410      & \bf 0.290      & \bf 0.394       & \bf 0.282      \\
\midrule
PRISM       & 0.114      & 0.024      & 0.178      & 0.124      & 0.131      & 0.084      & 0.089      & 0.064      & -0.040     & -0.040     & 0.094       & 0.051      \\
BLEURT-20   & 0.509      & 0.371      & 0.296      & 0.300      & 0.409      & 0.286      & 0.496      & 0.390      & 0.491      & 0.374      & 0.440       & 0.344      \\

COMET-QE-DA 
& 0.417 & 0.324 
& 0.535 & \bf 0.404
& 0.551 & 0.430
& 0.386 & 0.341
&0.531 & 0.391 
& 0.414 & 0.378\\


COMET-QE-MQM 
& 0.387 & 0.309
& 0.590 & 0.403
& 0.577 & 0.392 
& 0.438 & 0.392
& 0.571 & 0.399
& 0.513 & 0.379
\\

COMET-DA    & \bf 0.557     & \bf 0.403     & \bf 0.581     & 0.390     &  0.426    &  0.306      & \textbf{0.531}      & \textbf{0.419}      &  0.529      &  0.412      & 0.525      & 0.386      \\

COMET-MQM   & 0.465    & 0.360      & 0.529      &   0.370    &  \bf 0.686     &  \bf 0.459   & 0.508       &   0.392    & \bf 0.597     & \bf  0.432    & \bf 0.557      & \bf 0.402     \\

% Indic-COMET-MQM        &  0.548      & \bf 0.420     & \bf 0.631      & \bf 0.426    & \bf 0.471         & \bf 0.332   &  0.502      &  0.409     & \bf 0.590      & \bf 0.447     \\
\bottomrule
\end{tabular}
}
\caption{Segment-level Pearson ($\rho$) and Kendall tau ($\tau$) correlations of different metrics. The best metric correlation amongst each metric category \cite{sai2022survey} in \textbf{bold}. We observe that COMET-MQM is the best-performing metric overall for all languages in consideration. All correlations are significant ($p< 0.05$). }
\label{tab:corr_formula_metrics}
\end{table*}
